Triple Overlap in Pipelined Krylov Methods on Multi-GPU Systems

We introduce a novel triple-overlap implementation of the pipelined preconditioned conjugate gradient (Pipe-PCG) and pipelined stabilized biconjugate gradient (Pipe-BiCGStab) solvers, methods widely used in scientific applications. By leveraging a collective communication library, our approach extends conventional computation-communication overlap to concurrently execute collective operations, irregular P2P communication, and compute kernels, enabling computation-communication-communication overlap across multiple GPUs. We evaluate the design on the MareNostrum 5 (H100) and Leonardo (A100) supercomputers, comparing against PETSc and the state-of-the-art two-stream NCCL implementation using SuiteSparse matrices and three massive instances scaled up to 512 GPUs. The three-stream design outperforms the two-stream baseline on every instance, with the margin widening from 2-6% at 4 GPUs to 18-47% at 64 GPUs. At 64 GPUs, the geometric-mean speedup over the two-stream baseline is 1.33x on MareNostrum 5 and 1.23x on Leonardo for Pipe-PCG, and reaches 1.30x for Pipe-BiCGStab. In large-scale experiments, we observed a speedup up to 35% in Pipe-PCG and up to 33% in Pipe-BiCGStab compared to the two-stream design. For PETSc, the margin is even wider, up to 3.27x speedup in both Pipe-PCG and Pipe-BiCGStab. Related code for the proposed method is available online: https://github.com/ParCoreLab/aCG

==> tables/MN5_allreduce.tex <==
\begin{comment}

---

## NCCL 2.24.3 — AllReduce Latency (16 B, double precision, in-place)

Collective: `all_reduce`, operation: `sum`, message size: 16 bytes (2 × `double`).
Each rank owns 1 GPU; 4 GPUs per node.

\end{comment}

\begin{table}
    \centering
    \begin{tabular}{rrrr}
    \toprule
    Nodes & No. of GPUs & Size [B] & Latency [µs] \\
    \midrule
    1  & 4   & 16 & 8.32  \\
    2  & 8   & 16 & 16.36 \\
    4  & 16  & 16 & 24.82 \\
    8  & 32  & 16 & 33.01 \\
    16 & 64  & 16 & 45.43 \\
    \bottomrule
    \end{tabular}
    \caption{Latency (in microseconds) of an \texttt{ncclAllReduce} operation reported by the {\ttfamily nccl-tests} benchmarks on MareNostrum~5 
    %using NCCL~2.24.3 
    for a 16-byte message (two double-precision values) using in-place reduction.}
    \label{tab:marenostrum5_allreduce}
\end{table}


\begin{comment}

| GPUs | Nodes | In-place Latency [µs] |
|------|-------|----------------------|
| 4    | 1     | 8.32                 |
| 8    | 2     | 16.36                |
| 16   | 4     | 24.82                |
| 32   | 8     | 33.01                |
| 64   | 16    | 45.43                |
| 128  | 32    | pending              |
| 256  | 64    | pending              |
\end{comment}

==> tables/MN5_p2p.tex <==
%
% nccl-tests sendrecv_perf results from MareNostrum5
%
\begin{table}
    \centering
    \begin{tabular}{rrr}
    \toprule
    Size [B] & Throughput [MB/s] & Latency [µs] \\
    \midrule
        1,024 &     47.4 &   21.59 \\
        2,048 &     95.6 &   21.42 \\
        4,096 &    189.3 &   21.63 \\
        8,192 &    369.0 &   22.20 \\
       16,384 &    648.6 &   25.26 \\
       32,768 &  1,198.1 &   27.35 \\
       65,536 &  1,982.9 &   33.05 \\
      131,072 &  3,557.9 &   36.84 \\
      262,144 &  6,358.1 &   41.23 \\
      524,288 &  9,271.2 &   56.55 \\
    1,048,576 & 12,979.0 &   80.79 \\
%    2,097,152 & 15,737.3 & 133.26 \\
%    4,194,304 & 17,705.7 & 236.89 \\
    \bottomrule
    \end{tabular}
    \caption{Throughput (in MB/s) and latency (in microsecs) of internode point-to-point communication with \texttt{ncclSend}/\texttt{ncclRecv} with different message sizes, as reported by the \texttt{nccl-tests} benchmarks on 2 H100 GPUs on MareNostrum5. (Theoretical max bandwidth is 25 GB/s.)}
    \label{tab:marenostrum5_p2p}
\end{table}

% ========================================
% Job: 38703199  Nodes: as01r2b[21,26]
% Date: Wed Apr  8 21:50:56 CEST 2026
% ========================================
% 0, NVIDIA H100, 65247 MiB
% 1, NVIDIA H100, 65247 MiB
% 2, NVIDIA H100, 65247 MiB
% 3, NVIDIA H100, 65247 MiB
% # nccl-tests version 2.18.2 nccl-headers=22403 nccl-library=22403
% # Collective test starting: sendrecv_perf
% # nThread 1 nGpus 1 minBytes 8 maxBytes 4294967296 step: 2(factor) warmup iters: 5 iters: 20 agg iters: 1 validation: 1 graph: 0 unalign: 0
% #
% # Using devices
% #  Rank  0 Group  0 Pid  30727 on  as01r2b21 device  0 [0000:1b:00] NVIDIA H100
% #  Rank  1 Group  0 Pid 1638636 on  as01r2b26 device  0 [0000:1b:00] NVIDIA H100
% NCCL version 2.24.3+cuda12.2
% #
% #                                                              out-of-place                       in-place          
% #       size         count      type   redop    root     time   algbw   busbw  #wrong     time   algbw   busbw  #wrong 
% #        (B)    (elements)                               (us)  (GB/s)  (GB/s)             (us)  (GB/s)  (GB/s)         
%            8             1    double     sum      -1    22.30    0.00    0.00       0    21.67    0.00    0.00    N/A
%           16             2    double     sum      -1    21.36    0.00    0.00       0    21.20    0.00    0.00    N/A
%           32             4    double     sum      -1    21.32    0.00    0.00       0    21.22    0.00    0.00    N/A
%           64             8    double     sum      -1    21.29    0.00    0.00       0    21.18    0.00    0.00    N/A
%          128            16    double     sum      -1    21.18    0.01    0.01       0    21.33    0.01    0.01    N/A
%          256            32    double     sum      -1    21.53    0.01    0.01       0    21.48    0.01    0.01    N/A
%          512            64    double     sum      -1    21.37    0.02    0.02       0    21.32    0.02    0.02    N/A
%         1024           128    double     sum      -1    21.59    0.05    0.05       0    21.42    0.05    0.05    N/A
%         2048           256    double     sum      -1    21.42    0.10    0.10       0    21.31    0.10    0.10    N/A
%         4096           512    double     sum      -1    21.63    0.19    0.19       0    21.56    0.19    0.19    N/A
%         8192          1024    double     sum      -1    22.20    0.37    0.37       0    21.88    0.37    0.37    N/A
%        16384          2048    double     sum      -1    25.26    0.65    0.65       0    25.25    0.65    0.65    N/A
%        32768          4096    double     sum      -1    27.35    1.20    1.20       0    27.07    1.21    1.21    N/A
%        65536          8192    double     sum      -1    33.05    1.98    1.98       0    32.96    1.99    1.99    N/A
%       131072         16384    double     sum      -1    36.84    3.56    3.56       0    36.80    3.56    3.56    N/A
%       262144         32768    double     sum      -1    41.23    6.36    6.36       0    39.79    6.59    6.59    N/A
%       524288         65536    double     sum      -1    56.55    9.27    9.27       0    55.85    9.39    9.39    N/A
%      1048576        131072    double     sum      -1    80.79   12.98   12.98       0    80.30   13.06   13.06    N/A
%      2097152        262144    double     sum      -1   133.26   15.74   15.74       0   132.67   15.81   15.81    N/A
%      4194304        524288    double     sum      -1   236.89   17.71   17.71       0   236.69   17.72   17.72    N/A
%      8388608       1048576    double     sum      -1   444.92   18.85   18.85       0   444.51   18.87   18.87    N/A
%     16777216       2097152    double     sum      -1   861.50   19.47   19.47       0   860.03   19.51   19.51    N/A
%     33554432       4194304    double     sum      -1  1691.24   19.84   19.84       0  1689.19   19.86   19.86    N/A
%     67108864       8388608    double     sum      -1  3350.83   20.03   20.03       0  3350.40   20.03   20.03    N/A
%    134217728      16777216    double     sum      -1  6670.26   20.12   20.12       0  6670.49   20.12   20.12    N/A
%    268435456      33554432    double     sum      -1  13309.7   20.17   20.17       0  13316.6   20.16   20.16    N/A
%    536870912      67108864    double     sum      -1  26589.5   20.19   20.19       0  26587.8   20.19   20.19    N/A
%   1073741824     134217728    double     sum      -1  53139.2   20.21   20.21       0  53156.5   20.20   20.20    N/A
%   2147483648     268435456    double     sum      -1   106272   20.21   20.21       0   106270   20.21   20.21    N/A
%   4294967296     536870912    double     sum      -1   212463   20.22   20.22       0   212497   20.21   20.21    N/A
% # Out of bounds values : 0 OK
% # Avg bus bandwidth    : 8.99309 
% #
% # Collective test concluded: sendrecv_perf
% #


% Job finished: Wed Apr  8 21:51:25 CEST 2026

